Hybrid Instance-aware Temporal Fusion for Online Video Instance Segmentation

Recently, transformer-based image segmentation methods have achieved notable success against previous solutions. While for video domains, how to effectively model temporal context with the attention of object instances across frames remains an open problem. In this paper, we propose an online video instance segmentation framework with a novel instance-aware temporal fusion method. We first leverages the representation, i.e., a latent code in the global context (instance code) and CNN feature maps to represent instance- and pixel-level features. Based on this representation, we introduce a cropping-free temporal fusion approach to model the temporal consistency between video frames. Specifically, we encode global instance-specific information in the instance code and build up inter-frame contextual fusion with hybrid attentions between the instance codes and CNN feature maps. Inter-frame consistency between the instance codes are further enforced with order constraints. By leveraging the learned hybrid temporal consistency, we are able to directly retrieve and maintain instance identities across frames, eliminating the complicated frame-wise instance matching in prior methods. Extensive experiments have been conducted on popular VIS datasets, i.e. Youtube-VIS-19/21. Our model achieves the best performance among all online VIS methods. Notably, our model also eclipses all offline methods when using the ResNet-50 backbone.

==> method.tex <==
\cb{
\section{Method}

\subsection{}

\subsection{Frame Representation}
Inspired by MaX-DeepLap~\cite{}, we unitize a global latent code as well as CNN feature maps to jointly represent instance-aware features of each frame, and further model correlation of frames using such representations. \ca{difference from MaxDeepLab.}

\paragraph{Instance code.}

\subsection{Instance-aware Correlation Modeling}
To model the frame-wise correlation at both instance level and pixel level, we build up corresponding attention layers based on transformer. Frame representations are further enhanced by leveraging such correlation modeling. 

\subsubsection{Intra-frame Attention}

\subsubsection{Inter-frame Attention}
Inter-frame attention aims to construct temporal correlation and fuse contextual feature across frames.



} % end of \cb
